Raising Secure Coding Awareness for Software Developers in the Industry

Many industrial IT security standards and policies mandate the usage of a secure coding methodology in the software development process. This implies two different aspects: first, secure coding must be based on a set of secure coding guidelines, and second software developers must be aware of these secure coding practices. On the one side, secure coding guidelines seems a bit like a black-art: while there exist abstract guidelines that are widely accepted, low-level secure coding guidelines for different programming languages are scarce. On the other side, once a set of secure coding guidelines is chosen, a good methodology is needed to make them known by the people which should be using them, i.e. software developers. Motivated both by the secure coding requirements from industry standards and also by the mandate to train staff on IT security by the global industry initiative "Charter of Trust", this paper presents an overview of important research questions on how to choose secure coding guidelines and on how to raise software developer awareness for secure coding using serious games.

==> tables/guidelines.tex <==
\begin{table*}[ht]
  \centering
  \caption{Secure Coding Guidelines}
  \label{tab:guidelines}
  \begin{tabular}{|p{2.4cm}|p{7cm}|p{0.7cm}|}
    \hline
      {\bf Name} & {\bf Publisher} & {\bf Year} \\
    \hline
      MISRA-C~\cite{MISRA_C:2012,MISRA_C_A1:2012} & Motor Industry Software Reliability Association & 2012 \\
    \hline
      WebAppSec~\cite{WWW_MOZILLA} & Mozilla & 2012 \\
    \hline
      OTGv4~\cite{WWW_OWASP_OTGv4} & Open Web Application Security Project & 2014 \\
    \hline
      SEI-C~\cite{WWW_SEI_C_2018} & Software Engineering Institute - Carnegie Mellon & 2018 \\
      SEI-C++~\cite{WWW_SEI_CPP_2018}  & & \\
      SEI-Java~\cite{WWW_SEI_JAVA_2018}  &  & \\
      SEI-Perl ~\cite{WWW_SEI_PERL_2018} & & \\
    \hline
      OWASP~\cite{owaspT10} & Open Web Application Security Project & 2017 \\
    \hline
  \end{tabular}
\end{table*}



==> tables/policy_vs_guideline.tex <==
\begin{table*}[ht]
  \centering
  \caption{Security Policy vs Secure Coding Guidelines}
  \label{tab:policy_vs_guideline}
  \begin{tabular}{|p{2cm}|p{7cm}|p{7cm}|}
    \hline
      & {\bf Security Policy} & {\bf Secure Coding Guideline} \\
    \hline
      Goal 
      & 
      Establish the company’s strategy to deal with information security aligned with business objectives
      &
      Establish the company’s strategy on how to write secure software aligned with best known secure software development practices \\
    \hline
      Controling
      &
      Organization actively controls and monitors the application of policies
      &
      Application of secure coding guidelines is delegated to compiled software; no monitoring is possible
      \\
    \hline
      Exceptions
      &
      Exceptions can be allowed if benefits outweigh the risks
      &
      In general, no exceptions allowed, otherwise a vulnerability is being introduced into the source code
      \\
    \hline
      Protection Goals
      &
      Confidentiality, Integrity, Availability of Business, Customers, Partners
      &
      Confidentiality, Integrity, Availability of Data and Infrastructure
      \\
    \hline
      How to protect
      &
      Behavioral change on procedures
      &
      Behavioral change in writing software
      \\
    \hline
      Temporal aspect
      &
      Dynamic (e.g. if risk appetite is changed)
      &
      Static (compiled binary code cannot change)
      \\
    \hline
      Dissemination
      &
      Circulars, Infotainment, Posters, Security Awareness Training
      &
      Documentation, Training
      \\
    \hline
      Enforcement
      &
      Administrative, Technical, Physical Processes and Controls 
      &
      Code Reviews, Static Code Analysis, Secure Software Tests
      \\
    \hline
  \end{tabular}
\end{table*}



==> tables/standards.tex <==
\begin{table}[ht]
  \centering
  \caption{Industrial Security Standards}
  \label{tab:standards}
  \begin{tabular}{|C{1.4cm}|p{6cm}|}
    \hline
      {\bf Name} & {\bf Publisher} \\
    \hline
      NIST SP 800 series& National Institute of Standards and Technology \\
    \hline
      62.443 & International Electrotechnical Commission \\
    \hline
      2700x & International Standards Organization \\
    \hline
      PCI/DSS & PCI Security Standards Council \\
    \hline
      B 5.21 & Bundesamt für Sicherheit in der Informationstechnik \\
    \hline
      ISO/IEC TR 24731-1 & International Electrotechnical Commission \\
    \hline
      BDEW & Bundesverband der Energie- und Wasserwirtschaft e.V \\
    \hline
      C2M2: Cybersecurity Capability Maturity Model & U.S. Department of Homeland Security \\
    \hline
  \end{tabular}
\end{table}


